Your Diffusion Model is Secretly a Certifiably Robust Classifier

Generative learning, recognized for its effective modeling of data distributions, offers inherent advantages in handling out-of-distribution instances, especially for enhancing robustness to adversarial attacks. Among these, diffusion classifiers, utilizing powerful diffusion models, have demonstrated superior empirical robustness. However, a comprehensive theoretical understanding of their robustness is still lacking, raising concerns about their vulnerability to stronger future attacks. In this study, we prove that diffusion classifiers possess $O(1)$ Lipschitzness, and establish their certified robustness, demonstrating their inherent resilience. To achieve non-constant Lipschitzness, thereby obtaining much tighter certified robustness, we generalize diffusion classifiers to classify Gaussian-corrupted data. This involves deriving the evidence lower bounds (ELBOs) for these distributions, approximating the likelihood using the ELBO, and calculating classification probabilities via Bayes' theorem. Experimental results show the superior certified robustness of these Noised Diffusion Classifiers (NDCs). Notably, we achieve over 80% and 70% certified robustness on CIFAR-10 under adversarial perturbations with \(\ell_2\) norms less than 0.25 and 0.5, respectively, using a single off-the-shelf diffusion model without any additional data.

==> sections/abstract.tex <==
% % weak abstract 
% \begin{abstract}
% Diffusion models are recently employed as generative classifiers for robust classification. However, a comprehensive theoretical understanding of the robustness of diffusion classifiers is still lacking, leading us to question whether they will be vulnerable to future stronger attacks. In this study, we propose a new family of diffusion classifiers, named Noised Diffusion Classifiers~(NDCs), that possess state-of-the-art certified robustness. Specifically, we generalize the diffusion classifiers to classify Gaussian-corrupted data by deriving the evidence lower bounds (ELBOs) for these distributions, approximating the likelihood using the ELBO, and calculating classification probabilities via Bayes' theorem. We integrate these generalized diffusion classifiers with randomized smoothing to construct smoothed classifiers possessing non-constant Lipschitzness. Experimental results demonstrate the superior certified robustness of our proposed NDCs. Notably, we achieve 80\%+ and 70\%+ certified robustness on CIFAR-10 under adversarial perturbations with $\ell_2$ norm less than 0.25 and 0.5, respectively, using a single off-the-shelf diffusion model without any additional data.
% \end{abstract}



% abstract, the real motivation and real contribution
\begin{abstract}
% Diffusion models have recently been employed as generative classifiers for robust classification. However, a comprehensive theoretical understanding of the robustness of diffusion classifiers is still lacking, leading us to question whether they will be vulnerable to future stronger attacks. 
% In this study, we prove that diffusion classifiers possess \(O(1)\) Lipschitzness and obtain their certified robustness, demonstrating their inherent robustness. 
% To achieve a non-constant Lipschitzness (and thus a much tighter certified robustness), we generalize diffusion classifiers to classify Gaussian-corrupted data by deriving the evidence lower bounds (ELBOs) for these distributions, approximating the likelihood using the ELBO, and calculating classification probabilities via Bayes' theorem. 
% Experimental results demonstrate the superior certified robustness of these Noised Diffusion Classifiers (NDCs). Notably, we achieve over 80\% and 70\% certified robustness on CIFAR-10 under adversarial perturbations with \(\ell_2\) norms less than 0.25 and 0.5, respectively, using a single off-the-shelf diffusion model without any additional data.
Diffusion models have recently been employed as generative classifiers for robust classification. However, a comprehensive theoretical understanding of the robustness of diffusion classifiers is still lacking, raising concerns about their vulnerability to stronger future attacks. In this study, we prove that diffusion classifiers possess $O(1)$ Lipschitzness, and we establish their certified robustness, demonstrating their inherent resilience. To achieve non-constant Lipschitzness, thereby obtaining much tighter certified robustness, we generalize diffusion classifiers to classify Gaussian-corrupted data. This involves deriving the evidence lower bounds (ELBOs) for these distributions, approximating the likelihood using the ELBO, and calculating classification probabilities via Bayes' theorem. Experimental results show the superior certified robustness of these Noised Diffusion Classifiers (NDCs). Notably, we achieve over 80\% and 70\% certified robustness on CIFAR-10 under adversarial perturbations with \(\ell_2\) norms less than 0.25 and 0.5, respectively, using a single off-the-shelf diffusion model without any additional data.
\end{abstract}

==> sections/abstract_A.tex <==
% weak abstract 
\begin{abstract}
Diffusion models are recently employed as generative classifiers for robust classification. However, a comprehensive theoretical understanding of the robustness of diffusion classifiers is still lacking, leading us to question whether their robustness is overestimated. In this study, we fundamentally solve these concerns by deriving certified lower bounds of their robustness. We generalize them to classify any noisy data at any noise level by deriving the evidence lower bounds for noisy data distributions, approximating the likelihood using its lower bounds, and calculating classification probabilities via Bayes' theorem. We name these generalized diffusion classifiers as Noised Diffusion Classifiers~(NDCs), and construct smooth classifiers possessing non-constant Lipschitzness by combining NDCs with randomized smoothing, obtaining much higher certified robustness. Notably, we are the first to achieve 80\%+ and 70\%+ certified robustness on CIFAR-10 under adversarial perturbations with $\ell_2$ norm less than 0.25 and 0.5, respectively, using a single off-the-shelf diffusion model without any additional data.
\end{abstract}



% % stronger abstract
% \begin{abstract}
% Recent applications of diffusion models as generative classifiers for robust classification have shown promise, yet they lack theoretical underpinnings for their robustness    . In this work, we provide a unified framework for generative and discriminative modeling via diffusion models that possess certified lower bounds for their classification robustness. This framework approximates the log likelihood using evidence lower bounds and calculates classification probabilities through Bayes' theorem. 
% % We propose a new family of classifiers in this framework, named Noised Diffusion Classifiers, which can classify noisy data at any noise level, by deriving the Evidence Lower Bounds for noisy data distributions. 
% % Within this framework, we introduce an extension of diffusion classifiers, specifically designed to 
% We establish the Lipschitzness of generative models within this framework and determine their certified lower bounds for robust radii. Experimental results underscore the significant certified robustness of this new family of classifiers. Notably, this study is the first to achieve over 80\% and 70\% certified robustness on CIFAR-10 under $\ell_2$ norm-bounded adversarial perturbations of less than 0.25 and 0.5, respectively, employing only a single off-the-shelf diffusion model without the need for additional data.
% \end{abstract}


==> sections/intro.tex <==
\section{Introduction}

% \huanran{Current bug: Logic are not consistent

% -Abstract and method's logic: aims to theoretical analyze diffusion classifier.

% -Introduction and related work's logic: because diffusion classifier is good, we want to use diffusion model to construct certified classifier.

% }


Despite the unprecedented success of deep learning in the past decade \citep{lecun2015deep, openai2023gpt}, deep neural networks are vulnerable to adversarial examples, which are generated by imposing human-imperceptible perturbations to natural examples but can mislead a target model to make erroneous predictions \citep{szegedy2013intriguing, goodfellow2014explaining}. 
Adversarial examples pose a significant threat to real-world applications of deep learning, such as face recognition \cite{Sharif2016Accessorize,dong2019efficient}, autonomous driving \cite{cao2021invisible,jing2021too}, and the prevalent vision-language models \citep{carlini2023aligned,zhao2023evaluating,dong2023robust}. To improve model robustness, numerous defense techniques have been developed, including adversarial training \cite{pgd,zhang2019theoretically,rebuffi2021fixing_data_aug_improve_at}, input purification \cite{liao2018defense,nie2022diffpure}, adversarial example detection \cite{metzen2016detecting,pang2018towards}. 
% certified robustness~\cite{cohen2019certified,salman2019provably,hao2022gsmooth,carlini2022certified_diffpure_free}. 
However, there are still some limitations in existing methods. On the one hand, adversarial training requires more computational resources than standard training~\cite{adversarialMLAtScale,wong2020fast} and exhibits poor generalization against unseen threat models~\cite{tramer2019adversarial,nie2022diffpure}, limiting their applicability to real-world threats. On the other hand, due to the non-robust nature of discriminative classifiers, purification-based methods typically cannot completely purify adversarial perturbations, and thus their robustness lags behind the current state-of-the-art when defending against adaptive attacks~\cite{athalye2018obfuscated_gradient,lee2023robust,chen2023robust,kang2024diffattack}.



As a powerful family of generative models, diffusion models provide a more accurate estimation of the score function across the entire data space due to their generative nature. Consequently, diffusion models have recently been employed as generative classifiers for robust classification~\cite{li2023your,chen2023robust,clark2023text}. These classifiers are known as diffusion classifiers. Specifically, they calculate the classification probability \( p(y|\vect{x}) \propto p(\vect{x}|y) p(y) \) through Bayes' theorem and approximate the log likelihood \( \log p(\vect{x}|y) \) via the evidence lower bound (ELBO). This method establishes a connection between robust classification and the fast-growing field of pre-trained generative models. Although promising, there is still a lack of rigorous theoretical analysis, raising questions about whether their robustness is overestimated and whether they will be vulnerable to (potentially) stronger future adaptive attacks. In this work, we use theoretical tools to derive the certified robustness of diffusion classifiers, fundamentally address these concerns, and gain a deeper understanding of their robustness.





We begin by analyzing the smoothness of diffusion classifiers through the derivation of their Lipschitzness. We prove that diffusion classifiers possess an \(O(1)\) Lipschitz constant, demonstrating their inherent robustness. This allows us to certify the robust radius of diffusion classifiers by dividing the gap between predictions on the correct class and the incorrect class by their Lipschitz constant. Although we obtain a non-trivial certified radius, it could be much tighter if we could derive non-constant Lipschitzness (i.e., the Lipschitzness at each point). Randomized smoothing~\citep{cohen2019certified, salman2019provably}, a well-researched technique, allows us to obtain tighter Lipschitzness based on the output at each point. However, randomized smoothing requires the base classifier (e.g., diffusion classifiers) to process Gaussian-corrupted data \(\vect{x}_\tau\), where \(\tau\) is the noise level. To address this, we generalize diffusion classifiers to calculate \(p(y|\vect{x}_\tau)\) by estimating \(\log p(\vect{x}_\tau|y)\) using its ELBO and then calculating \(p(y|\vect{x}_\tau)\) using Bayes' theorem. We named these generalized diffusion classifiers as \textbf{Noised Diffusion Classifiers}. Hence, the core problem becomes deriving the ELBO for noisy data.





Naturally, we conceive to generalize the ELBO in \citet{sohl2015deep} and \citet{kingma2021variational_diffusion} to \(\tau \neq 0\), naming the corresponding diffusion classifier the Exact Posterior Noised Diffusion Classifier (EPNDC). EPNDC achieves state-of-the-art certified robustness among methods that do not use extra data. Surprisingly, we discover that one can calculate the expectation or ensemble of this ELBO without any additional computational overhead. This finding allows us to design a new diffusion classifier that functions as an ensemble of EPNDC but does not require extra computational cost. We refer to this enhanced diffusion classifier as the Approximated Posterior Noised Diffusion Classifier (APNDC). 
% Towards the end of this paper, we further reduce time complexity and enhance the scalability of diffusion classifiers for large datasets by using the same noisy samples for all classes to reduce variance. Additionally, we design a search algorithm to exclude as many candidate classes as possible at the outset of classification via a few samples.
Towards the end of this paper, we reduce the time complexity of diffusion classifiers by significantly decreasing variance through the use of the same noisy samples for all classes and by proposing a search algorithm to narrow down the candidate classes for the diffusion classifier.



Experimental results substantiate the superior performance of our methods. Notably, we achieve 82.2\%, 70.7\%, and 54.5\% at $\ell_2$ radii of 0.25, 0.5, and 0.75, respectively, on the CIFAR-10 dataset. These results surpass the previous state-of-the-art \cite{xiao2022densepure} by absolute margins of 5.6\%, 6.1\%, and 4.1\% in the corresponding categories. Additionally, our approach registers a clean accuracy of 91.2\%, outperforming \citet{xiao2022densepure} by 3.6\%. Moreover, our time complexity reduction techniques decrease the computational burden by a factor of 10 on CIFAR-10 and by a factor of 1000 on ImageNet, without compromising certified robustness. Furthermore, our comparative analysis with heuristic methods not only highlights the tangible benefits of our theoretical advancements but also provides valuable insights into several evidence lower bounds and the inherent robustness of diffusion classifiers.

The contributions of this paper are summarized as follows:

\begin{itemize}
\item We derive the Lipschitz constant and certified lower bound for diffusion classifiers, demonstrating their inherent provable robustness.
\item We generalize diffusion classifiers to classify noisy data, enabling us to derive non-constant Lipschitzness and state-of-the-art certified robustness.
\item We propose a variance reduction technique that greatly reduces time complexity without compromising certified robustness.
\end{itemize}




==> sections/intro_A.tex <==
\section{Introduction}

% \huanran{Current bug: Logic are not consistent

% -Abstract and method's logic: aims to theoretical analyze diffusion classifier.

% -Introduction and related work's logic: because diffusion classifier is good, we want to use diffusion model to construct certified classifier.

% }


Despite the unprecedented success of deep learning in the past decade \citep{lecun2015deep, openai2023gpt}, deep neural networks are vulnerable to adversarial examples, which are generated by imposing human-imperceptible perturbations to natural examples but can mislead a target model to make erroneous predictions \citep{szegedy2013intriguing, goodfellow2014explaining}. These adversarial examples pose a significant threat to real-world applications of deep learning, such as face recognition \cite{Sharif2016Accessorize,dong2019efficient}, autonomous driving \cite{cao2021invisible,jing2021too}, and even the advanced vision-language models \citep{carlini2023aligned,zhao2023evaluating,dong2023robust}. To improve model robustness, numerous defense techniques have been developed, including adversarial training \cite{pgd,zhang2019theoretically,rebuffi2021fixing_data_aug_improve_at}, input purification \cite{liao2018defense,nie2022diffpure}, adversarial example detection \cite{metzen2016detecting,pang2018towards}. However, most of these empirical defenses lack theoretical guarantees and can be further evaded by stronger adaptive attacks \cite{athalye2018obfuscated_gradient,tramer2020adaptive}. 


%Researchers have extensively explored defenses against adversarial examples, predominantly focusing on empirical methods, where the robustness of these methods is evaluated through adversarial attacks. For example, adversarial training, incorporating adversarial examples in training, has emerged as a dominant empirical defense in recent years~\citep{pgd,wang2023better_diffusion_improve_AT}. However, these empirical defenses lack theoretical guarantees and may be vulnerable to stronger future attacks.
In contrast, certified defenses \cite{raghunathan2018certified,sinha2018certifying,wong2018provable,cohen2019certified} have been proposed to provide a certified radius for an input such that the model's predictions are guaranteed to be unchanged for perturbations bounded by the radius. 
Among them, randomized smoothing \cite{cohen2019certified, hao2022gsmooth} is a model-agnostic approach scalable to large networks and datasets. It constructs a smoothed classifier that classifies an input image by taking the majority vote over the labels predicted by a base classifier under Gaussian noise of the input, which possesses non-constant Lipschitzness and thus has certified robustness. However, this method necessitates that the base model processes Gaussian-corrupted images, which poses a significant obstacle to its application in providing certified robustness for common classifiers.
% making the large collection of pre-trained models on clean data inapplicable and demanding additional computational overhead to train neural networks robust to Gaussian noise~\citep{cohen2019certified,salman2019provably, zhai2019macer}.

% Some recent work \cite{carlini2022certified_diffpure_free,xiao2022densepure} improves certified robustness of randomized smoothing by applying diffusion models \cite{sohl2015deep,ddpm,nichol2021improved,song2020score_diffusion_sde}, a powerful family of generative models, to denoise Gaussian-corrupted images due to their innate denoising nature. %diffusion models have been integrated into certified robustness frameworks. 
% In particular, \citet{carlini2022certified_diffpure_free} suggest using a diffusion model for one-step denoising of the inputs with Gaussian noise, followed by classification with a discriminative classifier. \citet{xiao2022densepure} further enhance this method by incorporating multiple denoising steps and advanced sampling techniques~\citep{ddim}. 
% % \citet{zhang2023diffsmooth} propose multiple cycles of denoising and noise addition to improve prediction consistency and, thus, certified robustness. 
% However, the success of these algorithms largely depends on the subsequent classifier, leading to a preference for large neural networks pre-trained on extensive datasets. 
% \hangx{Till now, the paragraph could be recognized as the background. In general, it is too long. Please get straight to the point, i.e., certified robustness and clarify the problem that this paper aims to address, to more swiftly dive into the main topic.}

Recently, \citet{chen2023robust} propose a new class of diffusion classifiers, which directly classify input images via an off-the-shelf diffusion model. The diffusion classifier calculates the classification probability $p(y|\vect{x}) \propto p(\vect{x}|y) p(y)$ through Bayes' theorem and approximates the log likelihood $\log p(\vect{x}|y)$ via its evidence lower bound (ELBO). This classifier achieves state-of-the-art empirical robustness across several types of threat models and can generalize to unseen attacks as it does not require training on adversarial examples. However, as a new type of classifier, there remain some concerns about its robustness evaluation. Critics question whether the robustness of this diffusion classifier has been largely overestimated by (potentially) insufficient evaluations. Although \citet{chen2023robust} conduct extensive analysis on its gradient randomness, magnitude, obfuscated gradients, and attack iterations, they still cannot completely dispel these doubts about diffusion classifiers. In this work, we aim to use theoretical tools to derive the certified lower bound for the robustness of diffusion classifiers, fundamentally address these concerns, and gain a deeper understanding of their robustness.

% due to the slight stochasticity of its gradient. Considering the diffusion models' dual capability to denoise and classify, we are prompted to ask: ``\textit{Is it possible to directly develop a \textbf{certifiably robust classifier} using \textbf{a single off-the-shelf diffusion model}?}''
% \hangx{what are the non-trivial challenges for the problem?}



We begin by analyzing the inherent smoothness of diffusion classifiers through the derivation of their Lipschitzness. However, the certified radius we obtain is not as tight as desired due to the assumption that the maximum Lipschitzness is maintained throughout the entire space. As a well-researched technique, randomized smoothing~\citep{cohen2019certified, salman2019provably} can derive non-constant Lipschitzness and thus a much larger certified robust radius. Therefore, to achieve a tighter certified radius, we integrate randomized smoothing, which necessitates that diffusion classifiers process Gaussian-corrupted data $\vect{x}_\tau$. Consequently, we propose \textbf{Noised Diffusion Classifiers}, which calculate $p(y|\vect{x}_\tau)$ from $\log p(\vect{x}_\tau|y)$ estimated by its ELBO. Hence, the problem turns to deriving the ELBO for noisy data. We first propose the Exact Posterior Noised Diffusion Classifier (EPNDC), which extends the ELBO in \citet{sohl2015deep} and \citet{kingma2021variational_diffusion} to \(\tau \neq 0\). Furthermore, we develop a better ELBO that is an expectation or ensemble of the first over all noisy samples derived from a single image but can be computed without incurring additional cost, and name corresponding diffusion classifier as Approximated Posterior Noised Diffusion Classifier (APNDC). In the end, we significantly reduce time complexity and enhance the scalability of diffusion classifiers for large datasets by using the same noisy samples for all classes to reduce variance and designing a search algorithm to exclude as many candidate classes as possible at the outset of classification via a few samples.


% Consequently, we derive two similar\junz{why care about two? what key difference?} ELBOs for the log likelihood of the corrupted data (i.e., $\log p(\vect{x}_\tau|y)$). The first is an extension of ELBO in \cite{sohl2015deep,ddpm,kingma2021variational_diffusion} for cases where \(\tau \neq 0\); the second is an expectation or ensemble of the first over all noisy samples derived from a single image, but can be computed without incurring additional cost. Based on these, we construct two \textbf{Noised Diffusion Classifiers} (\textbf{NDC}): the Exact Posterior Noised Diffusion Classifier (EPNDC) and the Approximated Posterior Noised Diffusion Classifier (APNDC), respectively, by $p(y|\vect{x}_\tau)\propto p(\vect{x}_\tau|y)p(y)$. Additionally, we propose several techniques that significantly reduce time complexity and enhance scalability to large datasets. 


Experimental results substantiate the superior performance of our methods. Notably, we establish new benchmarks in certified robustness, achieving $82.2\%$, $70.7\%$, and $54.5\%$ at $\ell_2$ radii of $0.25$, $0.5$, and $0.75$, respectively, on the CIFAR-10 dataset. These results surpass prior state-of-the-art~\cite{xiao2022densepure}, by margins of $5.6\%$, $6.1\%$, and $4.1\%$, in the corresponding categories. In addition, our approach registers a clean accuracy rate of $91.2\%$, outperforming \citet{xiao2022densepure} by $3.6\%$. Importantly, our time complexity reduction techniques reduce the computational burden by a factor of $10$ on CIFAR-10 and by an impressive factor of $1000$ on ImageNet. Remarkably, this substantial efficiency gain does not compromise the certified robustness of the model. Moreover, our comparative analysis with heuristic methods not only highlights the tangible benefits stemming from our theoretical advancements but also provides valuable theoretical insights into several evidence lower bounds and the inherent robustness of diffusion classifiers.




%Experimental results demonstrate the efficacy of our methods. Remarkably, we achieve certified robustness of \(82.2\%\), \(70.7\%\), and \(54.5\%\) at \(\ell_2\) radii of \(0.25\), \(0.5\), and \(0.75\), respectively, on the CIFAR-10 dataset, surpassing the previous state-of-the-art method~\citep{xiao2022densepure} by \(5.6\%\), \(6.1\%\), and \(4.1\%\), respectively. Our method also achieves a clean accuracy of \(91.2\%\), outperforming \citet{xiao2022densepure} by \(3.6\%\). The time complexity reduction techniques we propose reduce the time complexity by a factor of 10 on CIFAR-10 and 1000 on ImageNet, while still maintaining remarkable certified robustness. Furthermore, our comparison with the heuristic method not only underscores the practical impact of our theoretical contributions but also offers theoretical insights into the evidence lower bounds of noisy data and the robustness of diffusion classifiers.


==> sections/intro_su.tex <==
\section{Introduction}

% \huanran{Current bug: Logic are not consistent

% -Abstract and method's logic: aims to theoretical analyze diffusion classifier.

% -Introduction and related work's logic: because diffusion classifier is good, we want to use diffusion model to construct certified classifier.

% }


%Despite the unprecedented success of deep learning in the past decade \citep{lecun2015deep, openai2023gpt}, deep neural networks are vulnerable to adversarial examples, which are generated by imposing human-imperceptible perturbations to natural examples but can mislead a target model to make erroneous predictions \citep{szegedy2013intriguing, goodfellow2014explaining}. 
Adversarial examples pose a significant threat to real-world applications of deep learning, such as face recognition \cite{Sharif2016Accessorize,dong2019efficient}, autonomous driving \cite{cao2021invisible,jing2021too}, and the prevalent vision-language models \citep{carlini2023aligned,zhao2023evaluating,dong2023robust}. Although numerous empirical defense techniques have been developed to improve model robustness~\cite{pgd,zhang2019theoretically,rebuffi2021fixing_data_aug_improve_at, nie2022diffpure}, most of these defenses can be further evaded by stronger adaptive attacks \cite{athalye2018obfuscated_gradient,tramer2020adaptive}. 
%Researchers have extensively explored defenses against adversarial examples, predominantly focusing on empirical methods, where the robustness of these methods is evaluated through adversarial attacks. For example, adversarial training, incorporating adversarial examples in training, has emerged as a dominant empirical defense in recent years~\citep{pgd,wang2023better_diffusion_improve_AT}. However, these empirical defenses lack theoretical guarantees and may be vulnerable to stronger future attacks.
% In this case, certified defenses \cite{raghunathan2018certified,sinha2018certifying,wong2018provable,cohen2019certified} have been proposed to provide a certified radius for an input such that the model's predictions are guaranteed to be unchanged for perturbations bounded by the radius. 
% Among them, randomized smoothing \cite{cohen2019certified, hao2022gsmooth} is a model-agnostic approach scalable to large networks and datasets. It constructs a smoothed classifier that classifies an input image by taking the majority vote over the labels predicted by a base classifier under Gaussian noise of the input, which possesses non-constant Lipschitzness and thus has certified robustness. However, this method necessitates that the base model processes Gaussian-corrupted images, which poses a significant obstacle to its application in providing certified robustness for common classifiers.
To address these challenges, certified defenses \cite{raghunathan2018certified,sinha2018certifying,wong2018provable,cohen2019certified} have been proposed, which provide a certified radius for an input such that the model's predictions are guaranteed to remain unchanged for perturbations within that radius. Among these methods, randomized smoothing \cite{cohen2019certified,hao2022gsmooth} stands out as a model-agnostic approach scalable to large networks and datasets. It constructs a smoothed classifier that classifies an input image by taking the majority vote over the labels predicted by a base classifier under Gaussian noise of the input. This approach offers certified robustness due to its non-constant Lipschitzness. However, it necessitates that the base model processes Gaussian-corrupted images, leading to limitations such as small certified radii and high computational complexity, which pose significant obstacles to its application in providing certified robustness for common classifiers.
\hangx{the limitation should be consistent with the advantages in the experiments, e.g., small certified radius, high computational complexity }
% making the large collection of pre-trained models on clean data inapplicable and demanding additional computational overhead to train neural networks robust to Gaussian noise~\citep{cohen2019certified,salman2019provably, zhai2019macer}.

% Some recent work \cite{carlini2022certified_diffpure_free,xiao2022densepure} improves certified robustness of randomized smoothing by applying diffusion models \cite{sohl2015deep,ddpm,nichol2021improved,song2020score_diffusion_sde}, a powerful family of generative models, to denoise Gaussian-corrupted images due to their innate denoising nature. %diffusion models have been integrated into certified robustness frameworks. 
% In particular, \citet{carlini2022certified_diffpure_free} suggest using a diffusion model for one-step denoising of the inputs with Gaussian noise, followed by classification with a discriminative classifier. \citet{xiao2022densepure} further enhance this method by incorporating multiple denoising steps and advanced sampling techniques~\citep{ddim}. 
% % \citet{zhang2023diffsmooth} propose multiple cycles of denoising and noise addition to improve prediction consistency and, thus, certified robustness. 
% However, the success of these algorithms largely depends on the subsequent classifier, leading to a preference for large neural networks pre-trained on extensive datasets. 
% \hangx{Till now, the paragraph could be recognized as the background. In general, it is too long. Please get straight to the point, i.e., certified robustness and clarify the problem that this paper aims to address, to more swiftly dive into the main topic.}

\hangx{A steep transition to diffusion; why introduce diffusion to address certified defense? }Recently, various studies \cite{nie2022diffpure,carlini2022certified_diffpure_free} have applied diffusion models \cite{sohl2015deep,ddpm,song2020score_diffusion_sde} to improve the adversarial robustness, setting up  a connection between robust classification and the fast-growing field of pre-trained generative models. Notably, 
\citet{chen2023robust} propose a generative approach to achieve the state-of-the-art empirical robustness by constructing diffusion classifiers from pre-trained diffusion models. The diffusion classifiers calculate the classification probability $p(y|\vect{x}) \propto p(\vect{x}|y) p(y)$ through Bayes' theorem and approximate the log likelihood $\log p(\vect{x}|y)$ via the evidence lower bound (ELBO). 
%It set up a connection between robust classification and the fast-growing field of pre-trained generative models. Moreover, it has achieved state-of-the-art empirical robustness across several types of threat models and can generalize to unseen attacks as it does not require training on adversarial examples.   
Though promising, there is still lacking a rigorous theoretical analysis, leaving questions whether their robustness is being overestimated and whether they will be vulnerable to (potentially) future stronger adaptive attacks.
% However, as a new type of classifier, there remain some concerns about its robustness evaluation. Critics question whether their robustness is being overestimated and whether they will be vulnerable to (potentially) future stronger adaptive attacks. Although \citet{chen2023robust} conduct extensive analysis on its gradient randomness, magnitude, obfuscated gradients, and attack iterations, they still cannot completely dispel these doubts about diffusion classifiers. 
In this work, we use theoretical tools to derive the certified robustness of diffusion classifiers, fundamentally address these concerns, and gain a deeper understanding of their robustness.
\hangx{Actually, we introduce two different motivation, 1. certified defense and 2. whether diffusion classifier could be certified. better to follow a line}

% \junz{the following argument is kind-of too "personal" to RDC -- the critics exist for any empirically robust models, not just RDC or because of it is new; we should focus on the science -- the difference from empirical robustness vs. certified. Change to more general statements, e.g., "Though promising, it is still lacking a rigorous certified analysis, leaving questions whether they will be vulnerable to (potentially) future stronger adaptive attacks.". }


\hangx{we should rethink the logic. the current version is somewhat to apply random smoothing in diffusion classifier. In this case, it follow the second logic-line to some extent. We should clarify that what are the non-trivial challenges we have addressed?  }We begin by analyzing the inherent smoothness of diffusion classifiers through the derivation of their Lipschitzness. However, the certified radius we obtain is not as tight as desired due to the assumption that the maximum Lipschitzness is maintained throughout the entire space. As a well-researched technique, randomized smoothing~\citep{cohen2019certified, salman2019provably} can derive non-constant Lipschitzness and thus leads to a much larger certified robust radius. Therefore, to achieve a tighter certified radius, we integrate randomized smoothing, which necessitates that diffusion classifiers process Gaussian-corrupted data $\vect{x}_\tau$, where \(\tau\) is the noise level\hangx{it lead to an ``A+B'' paper. Be careful about such kind claim}. Consequently, we propose \textbf{Noised Diffusion Classifiers}, which calculate $p(y|\vect{x}_\tau)$ from $\log p(\vect{x}_\tau|y)$ estimated by its ELBO. Hence, the problem turns to deriving the ELBO for noisy data\hangx{what are the challenges?}. We first propose the Exact Posterior Noised Diffusion Classifier (EPNDC), which extends the ELBO in \citet{sohl2015deep} and \citet{kingma2021variational_diffusion} to \(\tau \neq 0\). Furthermore, we develop a better ELBO \hangx{better to what aspects? what are the limitation for the previous methods?} that is an expectation or ensemble of the first 
% over all noisy samples derived from a single image 
but can be computed without incurring additional cost, and name corresponding diffusion classifier as Approximated Posterior Noised Diffusion Classifier (APNDC). In the end, we significantly reduce time complexity and enhance the scalability of diffusion classifiers for large datasets by using the same noisy samples for all classes to reduce variance and designing a search algorithm to exclude as many candidate classes as possible at the outset of classification via a few samples.



Experimental results substantiate the superior performance of our methods. Notably, we establish new benchmarks in certified robustness, achieving 82.2\%, 70.7\%, and 54.5\% at $\ell_2$ radii of 0.25, 0.5, and 0.75, respectively, on the CIFAR-10 dataset. These results surpass the prior state-of-the-art \cite{xiao2022densepure} by absolute margins of 5.6\%, 6.1\%, and 4.1\% in the corresponding categories. Additionally, our approach registers a clean accuracy of 91.2\%, outperforming \citet{xiao2022densepure} by 3.6\%. Moreover, our time complexity reduction techniques decrease the computational burden by a factor of 10 on CIFAR-10 and by a factor of 1000 on ImageNet, without compromising certified robustness. Furthermore, our comparative analysis with heuristic methods not only highlights the tangible benefits of our theoretical advancements but also provides valuable insights into several evidence lower bounds and the inherent robustness of diffusion classifiers.


% Experimental results substantiate the superior performance of our methods. Notably, we establish new benchmarks in certified robustness, achieving $82.2\%$, $70.7\%$, and $54.5\%$ at $\ell_2$ radii of $0.25$, $0.5$, and $0.75$, respectively, on the CIFAR-10 dataset. These results surpass prior state-of-the-art~\cite{xiao2022densepure}, by absolute margins of $5.6\%$, $6.1\%$, and $4.1\%$, in the corresponding categories. In addition, our approach registers a clean accuracy of $91.2\%$, outperforming \citet{xiao2022densepure} by $3.6\%$. Moreover, our time complexity reduction techniques decrease the computational burden by a factor of 10 on CIFAR-10 and by a factor of 1000 on ImageNet, without compromising the certified robustness. Furthermore, our comparative analysis with heuristic methods not only highlights the tangible benefits stemming from our theoretical advancements but also provides valuable theoretical insights into several evidence lower bounds and the inherent robustness of diffusion classifiers.




%Experimental results demonstrate the efficacy of our methods. Remarkably, we achieve certified robustness of \(82.2\%\), \(70.7\%\), and \(54.5\%\) at \(\ell_2\) radii of \(0.25\), \(0.5\), and \(0.75\), respectively, on the CIFAR-10 dataset, surpassing the previous state-of-the-art method~\citep{xiao2022densepure} by \(5.6\%\), \(6.1\%\), and \(4.1\%\), respectively. Our method also achieves a clean accuracy of \(91.2\%\), outperforming \citet{xiao2022densepure} by \(3.6\%\). The time complexity reduction techniques we propose reduce the time complexity by a factor of 10 on CIFAR-10 and 1000 on ImageNet, while still maintaining remarkable certified robustness. Furthermore, our comparison with the heuristic method not only underscores the practical impact of our theoretical contributions but also offers theoretical insights into the evidence lower bounds of noisy data and the robustness of diffusion classifiers.

